Facial Surgery Preview Based on the Orthognathic Treatment Prediction

Orthognathic surgery consultation is essential to help patients understand the changes to their facial appearance after surgery. However, current visualization methods are often inefficient and inaccurate due to limited pre- and post-treatment data and the complexity of the treatment. To overcome these challenges, this study aims to develop a fully automated pipeline that generates accurate and efficient 3D previews of postsurgical facial appearances for patients with orthognathic treatment without requiring additional medical images. The study introduces novel aesthetic losses, such as mouth-convexity and asymmetry losses, to improve the accuracy of facial surgery prediction. Additionally, it proposes a specialized parametric model for 3D reconstruction of the patient, medical-related losses to guide latent code prediction network optimization, and a data augmentation scheme to address insufficient data. The study additionally employs FLAME, a parametric model, to enhance the quality of facial appearance previews by extracting facial latent codes and establishing dense correspondences between pre- and post-surgery geometries. Quantitative comparisons showed the algorithm's effectiveness, and qualitative results highlighted accurate facial contour and detail predictions. A user study confirmed that doctors and the public could not distinguish between machine learning predictions and actual postoperative results. This study aims to offer a practical, effective solution for orthognathic surgery consultations, benefiting doctors and patients.

==> cover_letter.tex <==
\thispagestyle{empty}
\noindent Dear \editorname,

Please find enclosed the revised version of our previous submission entitled \enquote{\thetitle} with manuscript number \manuscript. We would like to thank you and the reviewers for the valuable comments which help improving the quality of our manuscript.
In this revision, we have carefully addressed the reviewers' comments. A summary of the main modifications and a detailed point-by-point response to the comments from Reviewers (following the reviewers' order in the decision letter) are given below.

\vspace{8em}

\noindent Sincerely,

\noindent Huijun Han,  Congyi Zhang, Lifeng Zhu, Pradeep Singh, Richard Tai‑Chiu Hsung, Liu Yan Leung, Taku Komura, Wenping Wang, Min Gu
 


\vfill
\textbf{Note:} To enhance the legibility of this response letter, all the editor's and reviewers' comments are typeset in boxes. Rephrased or added sentences are typeset in color. The respective parts in the manuscript are highlighted to indicate changes.

==> reviewers/R1.tex <==
% Reviewer 1
\reviewer
\begin{revcomment}
Reproducibility: The description is quite clear, however, the dataset seems to be closed, therefore the study cannot be directly reproduced. 
\end{revcomment}
\begin{revresponse}[]


Thank you for your feedback. While we are unable to publicly share the facial scan dataset due to \textbf{ethical and privacy constraints}, we recognize the importance of reproducibility. 
To support further research, we plan to \textbf{release the implementation code}, allowing other researchers to apply our approach to their own datasets. 
Currently, the repository is private as we need some time to remove patient-specific data from the code. Once this is completed, we will make the repository publicly available at \href{https://github.com/ArchHazel/Orthognathics}{this github repository}. 
    
\end{revresponse}



\begin{revcomment}
Statistical analyses on user study: I suggest to improve Table 2 - the provided numbers (n=150 for medical professionals and n=450 for engineers) is not clear. Does it mean that such huge number of professionals answered the questionnaire or that it is the combined number of responses within the group? I assume that it is the second possibility - how many medical doctors and engineers answered the questionnaire? How were the cases selected? Randomly? With the lowest/largest quantitative error? This should be clarified in the Table description.
\end{revcomment}
\begin{revresponse}[]
Thank for pointing this out.  Accordingly, Table 2 has been revised.
\begin{changes}
\setcounter{table}{1} 
\hspace{-0.4cm}
\vbox{
\begin{table}[H]
\centering
\footnotesize
\begin{threeparttable}
\captionsetup{font=footnotesize}
\caption{ Comparison of Engineers' and Medical Professionals' ability to distinguish between Machine Learning-Generated faces and Real surgical outcomes}
\label{tab:statistical}

\begin{tabular}{lcc} 

\hline
 & \edit{Medical Professionals ($N_{med} = 5$) $n=150$ }& \edit{Engineers ($N_{eng}= 15$) $n=450$} \\
\hline
MLG & 34 (23\%) & 104 (23\%) \\
MLG identified as RSO & 41 (27\%) & 121 (27\%) \\
RSO identified as MLG & 35 (23\%) & 103 (23\%) \\
RSO & 40 (27\%) & 122 (27\%) \\

95\% CI & 12.58 to 17.02 &14.01 to 16.12\\ 
P-value  & 0.567 &0.256  \\
\hline
\end{tabular}
\begin{tablenotes}
\footnotesize
\item[] \edit{$N_{med}$, Number of medical professionals; $N_{eng}$, Number of engineers; n, number of responses; }
\item[] MLG, Machine learning generated faces; RSO, Real surgical outcomes; CI, Confidence Interval
\item[] McNemar chi-square test was performed unless otherwise mentioned.
\item[*] $p < 0.05$ (in \textbf{bold} \textit{italics}), considered statistically significant.
\end{tablenotes}
\end{threeparttable}
\end{table}
}
\end{changes}

As for the second part of reviewer’s concern, in our study, the patient images (cases) that participants assessed were selected randomly to ensure an unbiased and representative sample for evaluation. The selection process did not involve considerations of quantitative error, such as the magnitude of deviation or inaccuracy in the images. Instead, random selection was employed to minimize bias and enhance the generalizability of the findings. Therefore, the cases were chosen without regard to quantitative error, focusing on the random selection of patient images for assessment. To further clarify this, relevant section in the manuscript has been updated.

    \begin{changes}
A total of 30 randomly selected images (including A and B) were presented to each participant. 
    \end{changes}
\end{revresponse}



\begin{revcomment}
Statistical analyses on quantitative results: Yes, the interpretation and conclusions are supported by the data, however, all the quantitative differences are small. I suggest to add statistical analysis also to the ablation studies and to the comparison to LARS (Table 3, Table 4). 
\end{revcomment}
\begin{revresponse}[]
    Thank you for your suggestion. We have added statistical analysis to the ablation studies and the comparison with LARS in Tables 3 and 4. 
    Additionally, we have introduced a new table, which includes the statistical results showing significant differences between our method and LARS, with p-values less than 0.05.  This indicates that the differences observed are statistically significant, despite being small in magnitude.

    However, to conduct statistical experiments on the ablation study, we would need to further subdivide the patients, as not all patients require the facial asymmetry and mouth-convexity constraints. For those patients, the corresponding loss terms would not be significant. This would lead to a reduction in the test set size, making such an analysis difficult to perform. We hope this explanation clarifies why we have not included statistical analysis for ablation study in this context. In fact, we have provided qualitative examples demonstrating how incorporating these loss terms helps correct facial asymmetry and mouth protrusion. Please refer to Figure 5, specifically the first and second rows, for a visual illustration.
    
    \begin{changes}    
Table 5 presents the results of the statistical analysis
using a t-test to compare our model with the LARS model
based on two distance metrics: Hausdorff and Chamfer dis-
tances. The t-statistics and corresponding p-values indi-
cate that both metrics show statistically significant differ-
ences between the models. Specifically, for the Hausdorff
distance, our model demonstrated a t-statistic of 2.113
with a p-value of 0.039, which is below the 0.05 threshold
for significance. Similarly, for the Chamfer distance, the
t-statistic was 2.143 with a p-value of 0.036, also demon-
strating a significant difference. These results suggest that
our model outperforms the LARS model in terms of both
distance metrics.
\vbox{
\setcounter{table}{4} 
\begin{table}[H]
\centering
\captionsetup{font=small}
\caption{\edit{Statistical analysis of Hausdorff and Chamfer distances.}}
\begin{tabular}{llccl}
\hline
\textbf{Comparison}        & \textbf{Metric}   & \textbf{t-statistic} & \textbf{p-value} & \textbf{Significance} \\ \hline
Our model vs LARS model & Hausdorff         & 2.113               & 0.039            & Significant          \\ \hline
Our model vs LARS model & Chamfer           & 2.143               & 0.036            & Significant          \\ \hline
\end{tabular}

\label{tab:statistical_results}
\end{table}}
    \end{changes}
\end{revresponse}



\begin{revcomment}
    Limitation: the limitations are just briefly described in very short paragraph at the end of the article. I suggest to significantly expand the description of the limitations and their consequences.
\end{revcomment}

\begin{revresponse}[]
Thank you for your suggestion. We have revised the manuscript to significantly expand the description of the limitations and their consequences, providing a more detailed and thorough discussion towards the end of the article. 
\end{revresponse}
\begin{changes}
    Due to the unlabeled data used to train our network, our prediction model may not currently offer multimodal-based predictions for individual patients, considering factors such as age, gender, and skin condition. However, if additional data with multi-modal labels becomes available in the future, we could categorize the existing data by these factors, enabling us to make more targeted predictions without significantly reducing the data available for each category.

Our primary focus is on providing automatic visualization services for patients rather than serving orthognathic professionals, so we have not included adjustable parameters for doctors. In future work, if aiming to create a platform for medical professionals as surgical plans, we may consider incorporating user-friendly interfaces with adjustable parameters that offer semantic information.

Additionally, our model currently supports facial prediction primarily for Asian facial types, and further work will be needed to expand its applicability to other ethnic groups.
\end{changes}


\begin{revcomment}
   Highlight Character Limit: The highlights are too long. Elsevier does not allow such long highlights (the upper limit is up to 80 characters per highlight)
\end{revcomment}

\begin{revresponse}[]
Thank you for your comment. We have revised the highlights to adhere to the 80-character limit set by Elsevier.

\begin{changes}
    \begin{itemize}
        \item  { We propose an automated method for 3D post-surgical prediction using only multi view images.}

\item{We integrate mouth convexity and asymmetry criteria to enhance orthognathic planning.}

\item { We generate synthetic data from real cases to enhance training, improving robustness.}
    \end{itemize}
\end{changes}
\end{revresponse}


\begin{revcomment}
    The graphical abstract should not contain free text - it should be fully graphical. The purpose of the graphical abstract is to grasp the article idea without reading the detailed description.
\end{revcomment}

\begin{revresponse}[]
Thank you for your valuable feedback.
We have revised the graphical abstract accordingly.
\end{revresponse}

\begin{revcomment}
    How many different surgeons performed the orthognathic surgery for the collected dataset? It is quite important to give the information in order to discuss whether the heterogeneity of the surgery outcomes is sufficient. In case the number of surgeons is limited - it should be mentioned in the limitations because the network may learn features related strongly to particular surgeon.
\end{revcomment}

\begin{revresponse}[]
Thank you for raising this concern. In response to your query regarding the number of different surgeons who performed the orthognathic surgery for the collected dataset, we would like to clarify that a total of \textbf{35 different surgeons} were involved in conducting the surgeries included in our study. This information is essential as it contributes to the diversity and heterogeneity of the surgical outcomes in our dataset. By involving a significant number of surgeons in the dataset, we aimed to ensure that the machine learning model does not inadvertently learn features that are specific to any individual surgeon. This approach was implemented to facilitate a more comprehensive and generalized analysis of the surgical outcomes. We appreciate your attention to this detail, and we has ensured that this information is included in the dataset section of the study to provide transparency regarding the dataset's composition and address your concern effectively. 
\end{revresponse}

\begin{changes}
    A total of 163 pairs of pre- and post-operative 3D facial scans were collected using the 3dMD facial scan acquisition system from patients undergoing orthognathic surgery at the University of Hong Kong School of Dentistry, performed by a diverse group of 35 different surgeons.
\end{changes}


==> reviewers/R2.tex <==
% Reviewer 2
\reviewer

\begin{revcomment}\label{comment:work-not-good}
Objectives and rationale of the study: The objectives and rationale of the study are generally stated, but they could be further clarified and strengthened to improve reader comprehension and contextual relevance.
        
\end{revcomment}
\begin{revresponse}[]

Thank you for your review and feedback. While Reviewer \#1 considered the objectives to be clearly stated, we appreciate your suggestions and would like to take this opportunity to further clarify the objectives and rationale of our study.

To clarify our study’s rationale, orthognathic surgery consultations play a crucial role in helping patients understand how their facial appearance may change post-surgery. However, existing visualization methods often suffer from inefficiency and inaccuracy due to the limited availability of pre- and post-treatment data, as well as the complexity of the surgical procedures. Our study aims to address these challenges by developing a \textbf{fully automated pipeline} capable of generating accurate and efficient 3D previews of postsurgical facial appearances—\textbf{all without requiring additional medical images such as CBCT scans}. This approach enhances accessibility for patients and improves the visualization process, making it both more efficient and clinically useful.


\end{revresponse}

\begin{revcomment}
Reproducibility: The study provides a strong methodological foundation, but several areas require additional detail to enhance replicability and reproducibility. Below are specific suggestions for improvement.
\begin{itemize}
    \item The study does not provide access to the trained model, implementation code, or dataset, making it difficult for other researchers to reproduce results.
    \item The data augmentation scheme \textbf{modifies the lower face} while \textbf{keeping the upper face unchanged}, but there is no precise description of the augmentation techniques used (e.g., GAN-based, warping, random deformation).
    \item The manuscript states that 5-fold cross-validation was used but does not specify how patients were split (random shuffle vs. stratified by demographic factors).
\end{itemize}

\end{revcomment}
\begin{revresponse}[]
    Thanks for your comments.
    \begin{itemize}
        \item Reproducibility: We plan to  \textbf{release the code} to facilitate future research. This will allow other researchers to perform inference using their own datasets. By making these resources publicly available, we aim to support reproducibility in the research community.
        \item Data Augmentation Scheme: Our goal is to generate a pair of facial scans that reflect the pre- and post-surgery appearance. To achieve this, we modify the upper part of the face, while the lower part of the face is copied directly from the dataset, following the paired changes between the pre- and post-surgery scans. As a result, we obtain a pair of faces where the upper part remains consistent, while the lower part exhibits the surgical changes. In summary, in our study, the actual operation involves \textbf{modifying the upper part} of the face while \textbf{keeping the lower part consistent with the corresponding data in the dataset}. The reviewer may have misunderstood the approach.
           
We have added the following paragraph to further clarify and address the reviewer’s misunderstanding:

    \begin{changes}
    In summary, our goal is to generate paired facial scans that reflect the pre- and post-surgery appearance. We modify the upper part of the face while directly copying the lower part from the dataset, following the paired changes between the pre- and post-surgery scans. As a result, we obtain a pair of faces where the upper part remains consistent, and the lower part exhibits the surgical changes. 
    \end{changes}

    
        
        Specifically, we use a variant $\xi$ to alter the latent code of the upper face, and then we use the decoder to reconstruct the facial geometry. This approach does not involve GAN-based methods, warping, or direct deformation on the facial geometry.

    \begin{changes}
We use a variant 
$\xi$ to alter the latent code of the upper face, and then we use the decoder to reconstruct the facial geometry. 
    \end{changes}
    

        
        \item Data splitting: In our manuscript, we mentioned that the 163 valid pairs of facial scans were shuffled and split into 5 consecutive folds. To clarify, the term "shuffled" indicates that the data was randomly distributed into these folds. This means that the data was randomly mixed before being split, rather than being stratified by any specific demographic factors. We has updated the manuscript to specify that the split was done via random shuffle to ensure clear communication.


    \begin{changes}
    The 163 valid pairs of facial scans were subjected to random shuffle and then split into 5 consecutive folds for cross-validation.
    \end{changes}
        \end{itemize}




    
\end{revresponse}

\begin{revcomment}
Statistical analyses: The manuscript only reports p-values but does not include confidence intervals (CIs) or effect sizes, which are essential for interpreting the practical significance of findings. The manuscript states that the user study included 5 medical professionals (2 surgeons, 3 orthodontists) and 15 engineers, but does not explain how participants were selected.
The manuscript compares its model against LARS, but does not include a baseline control (e.g., manual surgeon-based soft tissue prediction). The study correctly uses McNemar’s test but does not explain why other tests (e.g., chi-square, paired t-tests) were not used. The manuscript states that the mean Hausdorff Distance was 9.00 mm, but does not explain whether this deviation is clinically acceptable.

\end{revcomment}

\begin{revresponse}[]

\textbf{Regarding Confidence Intervals}: We appreciate the reviewer's feedback and acknowledge the importance of providing confidence intervals (CIs) in research reporting to enhance the interpretation of study findings. In response to this valuable suggestion, we have included CIs in the revised Table 2 to provide a more comprehensive understanding of the practical significance of our results.
 \begin{changes}
\setcounter{table}{1} 
\hspace{-0.4cm}
\vbox{
\begin{table}[H]
\centering
\footnotesize
\begin{threeparttable}
\captionsetup{font=footnotesize}
\caption{ Comparison of Engineers' and Medical Professionals' ability to distinguish between Machine Learning-Generated faces and Real surgical outcomes}
\label{tab:statistical}

\begin{tabular}{lcc} 

\hline
 & Medical Professionals ($N_{med} = 5$) $n=150$ & Engineers ($N_{eng}= 15$) $n=450$\\
\hline
MLG & 34 (23\%) & 104 (23\%) \\
MLG identified as RSO & 41 (27\%) & 121 (27\%) \\
RSO identified as MLG & 35 (23\%) & 103 (23\%) \\
RSO & 40 (27\%) & 122 (27\%) \\

\edit{95\% CI} & \edit{12.58 to 17.02} &\edit{14.01 to 16.12}\\ 
P-value  & 0.567 &0.256  \\
\hline
\end{tabular}
\begin{tablenotes}
\footnotesize
\item[] $N_{med}$, Number of medical professionals; $N_{eng}$, Number of engineers; n, number of responses; 
\item[] MLG, Machine learning generated faces; RSO, Real surgical outcomes; \edit{CI, Confidence Interval}
\item[] McNemar chi-square test was performed unless otherwise mentioned.
\item[*] $p < 0.05$ (in \textbf{bold} \textit{italics}), considered statistically significant.
\end{tablenotes}
\end{threeparttable}
\end{table}
}
\end{changes}
\textbf{Regarding Participant Selection}: The selection process for participants in our study involved recruiting a total of five medical professionals, comprising two surgeons and three orthodontists, with a minimum of 5 years of experience in their respective fields. Additionally, 15 engineers were included in the study, each possessing a minimum of 3 years of relevant experience in engineering and technical disciplines. The selection criteria for medical professionals were based on their expertise in surgical procedures and orthodontic treatments, ensuring a minimum threshold of 5 years of clinical experience. Engineers were chosen for their technical background and familiarity with machine learning concepts, with a minimum of 3 years of professional experience in their respective fields. By incorporating years of experience as a criterion for participant selection, we aimed to ensure that individuals with substantial practical knowledge and expertise contributed to the assessment of differentiating between machine learning-generated faces and real surgical outcomes. Accordingly, this information has been updated in the revised manuscript to offer transparency and clarity regarding the composition of the study sample.
    \begin{changes}
    Participants in this study consisted of five medical professionals (comprising two surgeons and three orthodontists) with a minimum of 5 years of experience in their respective fields. Additionally, 15 engineers (including twelve males and three females) were included in the study, each possessing a minimum of 3 years of relevant experience in engineering and technical disciplines. The selection criteria for medical professionals were based on their expertise in surgical procedures and orthodontic treatments, ensuring a minimum threshold of 5 years of clinical experience. Engineers were chosen for their technical background and familiarity with machine learning concepts, with a minimum of 3 years of professional experience in their respective fields. 
    \end{changes}
\textbf{Regarding Baseline Control}: We did consider including a manual surgeon-based soft tissue prediction as a baseline control. However, we decided not to proceed with this comparison because \textbf{each surgeon's approach and preferences for manual adjustments can vary significantly}. This variability makes it difficult to interpret differences between our predicted results and those of manual adjustments as a clear indication of prediction accuracy. As a result, we chose not to include this experiment, as it may \textbf{introduce confounding factors} that could complicate the evaluation of our model's performance. Instead, we have provided real pre- and post-surgical facial changes as a reference, which we believe offers a more consistent and reliable basis for evaluating our model's performance.

\textbf{Regarding the Choice of Statistical Tests}: The decision to use McNemar's test in our study was based on the specific nature of our research design and the type of data we collected. \textbf{McNemar's test is specifically designed to analyze paired nominal data}, where each participant provides responses to two related conditions or variables (in our case, images A and B) in a dichotomous format (correct/incorrect). This test is particularly suited for assessing changes or differences in proportions within paired data, making it a suitable choice for our study design.
In contrast, chi-square tests are typically used to analyze the independence or association between two categorical variables in a cross-tabulation format, while paired t-tests are used for comparing the means of two related groups or conditions. Since our study focused on comparing proportions of correct responses within paired data rather than assessing associations between categorical variables or comparing mean differences, McNemar's test was deemed the most appropriate statistical test for our research objectives. By selecting McNemar's test, we aimed to accurately evaluate the differences in response patterns between the two conditions (images A and B) within our study sample.


\textbf{Regarding Clinical Acceptance}: Thank you for raising the question concerning the clinical acceptability of the mean Hausdorff Distance of 9.00 mm reported in our manuscript. In the context of our study, the assessment of the mean Hausdorff Distance of 9.00 mm was not based on clinical criteria or considerations. Our primary objective was to evaluate the performance of a machine learning algorithm in generating facial images that simulate surgical outcomes, using the Hausdorff Distance as a metric to quantify the similarity between the simulated images and real surgical results. While the clinical acceptability of a Hausdorff Distance value is typically determined by specific clinical requirements and the nature of the medical imaging task, it is important to emphasize that Hausdorff Distance focused on the technical evaluation of the algorithm rather than its clinical applicability. \textbf{The acceptance of the results by surgeons in the user study was based on their assessment of the visual similarity and realism of the simulated facial images compared to actual surgical outcomes, rather than a clinical validation of the Hausdorff Distance value.} Our study conducted comprehensive quantitative evaluations, demonstrating high prediction accuracy for our method compared to the state of the art techniques. The reported Hausdorff Distance of 9.00 mm highlighted the superior performance of our method in generating facial images that simulate surgical outcomes and showcased the robustness and efficacy of our approach. It is important to note that while the mean Hausdorff Distance of 9.00 mm serves as a quantitative measure of similarity between the simulated and real images, the overall performance of our method, as demonstrated by the comprehensive evaluations and statistical analyses, indicates the effectiveness and reliability of our approach in generating accurate facial predictions. The acceptance of our results by domain experts underscores the practical relevance and usability of our method in simulating surgical outcomes.

\end{revresponse}

\begin{revcomment}
\textbf{Figures and Tables}:
\begin{itemize}
    \item Add a heatmap visualization that shows error distribution across facial regions.
        \item Overlay error maps on actual 3D scans to highlight discrepancies.
\item  Add a confusion matrix for user study results, showing true positives, false positives, true negatives, and false negatives.
\item Figure 4 and Figure 5 Need Clearer Labels for Predicted vs. Real Outcomes
\end{itemize}
\end{revcomment}



\begin{revresponse}[]
   \textbf{ Regarding heatmap:} We apologize for any confusion caused by the caption in Figure 4 and Figure 5. To clarify, we have indeed included heatmaps in these figures that show the distribution of errors across facial regions. The columns labeled \textbf{ error map} display these heatmaps. Additionally, we have provided error bars to further illustrate the variability in the errors, which are shown in the bottom-right corner of the figure. We have also revised the figure captions accordingly for better clarity.
\begin{changes}
Figure 4: Comparison of our method with LARS across four patient cases. On the left, the ground truth (GT) pre- and post-surgical scans are shown for reference. The middle columns display our predicted results, and the right columns show the LARS model's predictions. To compare the prediction errors with the real outcomes, heatmaps are provided showing the error distribution across facial regions, with the error bars located in the bottom-right corner. 
\end{changes}
\begin{changes}
 Figure 5: Impact of losses and data augmentation on predictions.
The left section illustrates actual surgical data, the middle section presents results after removing specific modules, and the right section showcases the full-model predictions.
    \end{changes}
   
    \textbf{Regarding error map:} Regarding your request for overlaying error maps on actual 3D scans, our current approach of visualizing errors on predicted faces provides a similar insight, as it highlights the regions of the face where discrepancies occur. We believe that our method of marking the errors on predicted faces is more effective, as it allows us to show a more consistent visualization, particularly when comparing the prediction, error map, and prediction with texture. These visualizations convey the same information as the overlay on actual scans, but with clearer representation in the context of our study.

    \textbf{Regarding confusion matrix:} Thank you for your suggestion. Accordingly, Table 3 presenting TP, TN, FP and FN in confusion matrix has been included in the manuscript.

    \begin{changes}
    \vbox{\begin{table}[H]
    \centering
    \captionsetup{font=small}
    \begin{threeparttable}
 \edit{  \caption{\edit{Confusion matrix presenting True Positives, False Positives, True Negatives, and False Negatives.}}}
 \label{table:confusionMatric}
\begin{tabular}{clll}
\hline
\multicolumn{1}{l}{}                                                            &                    & \multicolumn{2}{l}{True Responses} \\ \hline
\multicolumn{1}{l}{}                                                            &                    & RSO              & MLG             \\ \cline{2-4} 
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Predicted \\ Responses\end{tabular}} & Predicted RSO\_med & 53.30\%          & 54.70\%         \\
                                                                                & Predicted MLG\_med & 46.70\%          & 45.30\%         \\
                                                                                & Predicted RSO\_eng & 54.20\%          & 53.80\%         \\
                                                                                & Predicted MLG\_eng & 45.80\%          & 46.20\%         \\ \hline


\end{tabular}
\begin{tablenotes}
% \centering
\footnotesize
\item[] RSO: Real surgical outcomes;
\item[] MLG: Machine learning-generated faces.
\end{tablenotes}
\end{threeparttable}

\end{table}}
    \end{changes}

    \textbf{Regarding clearer labels for predicted vs. real outcomes}: Thank you for your valuable suggestion. To improve clarity, we have updated the labels in Figures 4 and 5. All real outcomes are now labeled with \textbf{Real}, and all predicted outcomes are labeled with \textbf{Prediction}. Specifically, in Figure 4, the left columns are labeled as Preoperative Real Scan, Postoperative Real Scan, and Postoperative Scan with Texture, which represent the actual surgical data. The columns labeled Our Prediction, Our Error Map, and Our Prediction with Texture represent our results, while the columns labeled LARS Prediction, LARS Error Map, and LARS Prediction with Texture represent the LARS model results. 
    Similarly, in Figure 5, the left section includes the columns Preoperative Real Scan and Postoperative Real Scan, which represent the actual surgical data. The middle section consists of w/ Ablation Prediction and w/ Ablation Error Map, showcasing the results obtained after removing certain modules. The right section includes w/o Ablation Prediction and w/o Ablation Error Map, representing the predictions from the full model. 
    We hope this makes the distinction between predicted and real outcomes much clearer.


\end{revresponse}
\begin{revcomment}
    The study’s interpretation of results is mostly reasonable, but some conclusions are overstated or lack sufficient justification based on the data presented. The conclusion states that the method "has the potential to set new standards in pre-surgical visualization."
\end{revcomment}

\begin{revresponse}[]
    Thank you for your feedback. We modified the conclusion to make it more cautious and in line with the data presented.
   
\end{revresponse}

\begin{changes}
   The proposed method has the potential for practical application in pre-surgical visualization and aiding in decision-making.
\end{changes}

\begin{revcomment}
    The manuscript highlights several key strengths of the proposed 3D facial surgery prediction model, but some areas need further emphasis to better showcase the study’s novel contributions and practical advantages over existing methods.
\end{revcomment}

\begin{revresponse}[]
Thank you for your valuable comments. We list our key contributions as follow:
\begin{itemize}
    \item We integrate two carefully designed criteria, including minimizing mouth-convexity and minimizing asymmetry, into the machine learning procedure, specifically designed to align with the goals of orthognathic surgery, which enhances prediction accuracy and reflects the novelty of our approach.
    \item We devise an augmentation method to expand the available dataset, achieving more robust predictions.
    \item We complete a fully automated pipeline that showcases the postoperative changes in facial appearance to patients in 3D, which is a significant advantage as it does not require manually annotated data points or CBCT data.
\end{itemize}



\end{revresponse}



\begin{revcomment}
Limitation:
\begin{itemize}
    \item The study reports a mean Hausdorff Distance of 9 mm, but does not explain whether this level of error is clinically acceptable.
    \item The model is trained on pre- and post-operative facial scans from Asian patients, but soft tissue response to surgery varies between ethnicities due to differences in skin thickness, fat distribution, and skeletal structure.
    \item The model focuses on predicting facial soft tissue outcomes, but does not account for changes in underlying skeletal structures beyond the provided surgical plan. Bone remodeling, muscle adaptation, and long-term soft tissue settling are not factored into the predictions, which may affect long-term accuracy. 
    \item The study compares its model against LARS, but does not benchmark performance against expert surgeon-driven predictions.
\end{itemize}

\end{revcomment}



\begin{revresponse}[]
\textbf{Regarding Hausdorff distance}: please refer to Comment 2.3, where we discuss its clinical acceptance in more detail. We hope this clarifies your inquiry.

\textbf{Regarding Asian patients}: We added this to the limitations section that the model's effectiveness has only been validated on Asian patients. However, the algorithm is generalizable, and with additional data from other ethnicities, it can be retrained to adapt to those populations as well. 

\begin{changes}
    Additionally, our model currently supports facial prediction primarily for Asian facial types, and further work will be needed to expand its applicability to other ethnic groups.
\end{changes}
\textbf{
Regarding skeletal changes:
} Our primary goal is to provide predictions of facial soft tissue outcomes without the need for CBCT scans. Incorporating changes in underlying skeletal structures, such as bone remodeling, muscle adaptation, and long-term soft tissue settling, would indeed enhance the accuracy of long-term predictions. However, to account for these factors, CBCT data would be necessary. Since our focus is on achieving predictions without such data, we have not included skeletal changes in our model. 

\textbf{
Regarding surgeon-driven predictions:
} We recognize the importance of comparing our model against expert surgeon-driven predictions. However, we believe that surgeons' backgrounds and their individual surgical preferences can introduce additional variability into the comparison, making it a more complex and subjective benchmark. Different surgeons may prioritize different aspects of the surgery, which could influence their predictions. This adds more factors to the comparison, making it less straightforward. While we understand the value of such a benchmark, we focused on comparing our model to LARS as a more consistent reference.

    
\end{revresponse}

\begin{revcomment}
Structure:
\begin{itemize}
    \item The Introduction provides background information but does not clearly state the specific objectives of the study until later paragraphs. This affects the initial understanding of the study's purpose.
    \item The Methods section is quite dense and includes diverse components like data augmentation, model training, loss functions, and evaluation metrics without clear separation.
    \item The Discussion repeats some points mentioned in the Results and occasionally lacks a direct connection to the findings presented. There are redundant statements about the advantages of the model that could be streamlined.
\end{itemize}

\end{revcomment}

\begin{revresponse}
   \textbf{Regarding initial understanding: } We have revised the Introduction to clearly state the specific objectives of the study earlier in the text. The main objective, which is to develop a fully automated prediction tool for postsurgical facial appearance without the need for CBCT data, is now introduced upfront to improve the initial understanding of the study's purpose. 

   \begin{changes}
       Visualizing expected surgical outcomes has emerged as a crucial step in mitigating presurgical anxiety, setting realistic expectations, and improving overall patient satisfaction, particularly when CBCT data is not available.
   \end{changes}
   \textbf{Regarding method organization:} To enhance the clarity of the Methods section, we have added an introductory paragraph that outlines the key components of the method and their corresponding sections. 
   \begin{changes}
       The reconstructed 3D facial model is initially encoded into a latent code using FLAME~\cite{FLAME:SiggraphAsia2017}, a parametric facial model. A face predictor then estimates the difference between post- and pre-surgery facial features, guided by custom-tailored loss functions that specifically incorporate facial asymmetry and mouth-convexity rules relevant to orthognathic surgery (explained in Section 2.1). These rules are directly applied to the predicted facial geometry and back-propagated through the network in a differentiable manner (discussed in Section 2.3). To provide a fully textured post-treatment preview, we leverage the mesh coherence of the FLAME model, transferring the texture from pre-treatment 3D facial scans to the predicted face models (explained in Section 2.4). 
To address the challenge of limited training data, we introduce a novel data augmentation technique that significantly increases the number of face pairs, enhancing the robustness of the model (described in Section 2.2). 
The effectiveness of the predicted models is evaluated through a user study involving both medical professionals and engineers, with the robustness of the predictions assessed using McNemar’s test (outlined in Section 2.5).
   \end{changes}

   \textbf{Regarding discussion redundancy:} We have revised the Discussion to make it more concise and focused. Redundant statements about the advantages of the model have been streamlined.
   \begin{changes} Both quantitative (as shown in Table. 6) and qualitative (as shown in Figure. 5) results demonstrate their effectiveness.
   \end{changes}
   \begin{changes}
       
  The addition of augmented data appears to help reduce prediction error.
       \end{changes}
       \begin{changes}
Additionally, data augmentation seems to play an important role, as its absence introduces noticeable inconsistencies in facial predictions.
   \end{changes}
\end{revresponse}


\begin{revcomment}
  Lack of Clinical Validation for the Predicted Outcomes: The study evaluates 3D post-surgical facial prediction accuracy, but no actual clinical validation is performed.
The quantitative validation relies solely on Chamfer Distance and Hausdorff Distance, which measure geometric accuracy but do not confirm the clinical reliability of the predicted outcomes.

Problem: How well do the predicted facial outcomes align with actual patient satisfaction and clinical aesthetic standards?

Recommendation: The study should: Compare predicted results with actual patient feedback or clinician assessment.
Use additional evaluation metrics, such as soft-tissue analysis performed by maxillofacial surgeons.
\end{revcomment}

\begin{revresponse} []
Thank you for your comment on the clinical validation of our predicted outcomes. We understand that the Hausdorff Distance of 9.00 mm, while useful for geometric accuracy, does not fully reflect clinical reliability.

To address this, we have already conducted a user study, where the results were evaluated by surgeons based on the visual similarity and realism of the simulated facial images compared to actual surgical outcomes. This assessment was aimed at understanding the clinical acceptability of our method.

For detailed explanation, please refer to Comment 2.3.
    
\end{revresponse}

\begin{revcomment}
    Bias in the Dataset: The dataset consists of 163 patient scans, with a majority being of Asian descent.
    
    Problem: This limits the generalizability of the model to patients of different ethnic backgrounds with varying soft tissue properties.

Recommendation: Discuss the impact of dataset bias and whether ethnic variation affects prediction accuracy.
If the dataset is not diverse, acknowledge this as a limitation.

\end{revcomment}


\begin{revresponse}[]
    Thank you for your insightful comment.

The generalization of our model to diverse populations has not yet been tested, and this remains an open research question. We acknowledge that further experiments can be conducted using our model to evaluate its performance on different ethnic groups. It is important to note that our network is not specifically designed for Asian patients; the losses we incorporated, such as symmetry and facial convexity, are widely accepted in the medical field and can be applicable to various ethnicities.

We have also addressed this limitation in the manuscript, specifying that the model has only been tested on Asian patients so far.
\end{revresponse}


\begin{revcomment}
    Weak Statistical Interpretation in the User Study: The user study tested whether engineers and medical professionals could differentiate between machine-generated predictions and real surgical outcomes.
The study reports no statistically significant difference (p-values: 0.567 and 0.256) in their ability to distinguish between the two.

Problem: The conclusion drawn is misleading—low specificity ($\approx46\%$) suggests poor ability to distinguish predictions from reality, but this does not confirm clinical accuracy.
Recommendation: Instead of concluding that the model is "effective," acknowledge the limitations of subjective evaluation.
Include more detailed analysis of inter-rater variability.
\end{revcomment}

\begin{revresponse}[]
    Thank you for your thoughtful feedback on our study. We appreciate your attention to detail and the concerns raised regarding the statistical interpretation in the user study. Upon further consideration and in light of the study's aim to evaluate the realism and accuracy of the machine-generated faces, we believe that the inability of participants to distinguish between MLG faces and RSO may actually indicate the success of the machine learning model in producing realistic predictions. This suggests that the high level of realism in the generated images could have contributed to the lack of statistical significance in differentiating between the two categories.
 
We appreciate your suggestion regarding the importance of acknowledging the limitations of subjective evaluation. However, in response to your concern, we would like to emphasize the diverse composition of participants in our study, which included medical professionals (surgeons and orthodontists) and engineers with varied backgrounds. This diversity allowed for a comprehensive evaluation of the machine-generated faces, considering a range of perspectives and expertise. The inclusion of participants with different perceptions and experiences enhanced the robustness of the subjective evaluation process and provided valuable insights into the realism and accuracy of the generated facial images. Given the strengths of the diverse participant composition in contributing to a more holistic assessment of the machine learning model's performance, we believe that the subjective evaluation, in this context, may not be considered a significant limitation. The varied viewpoints and expertise of the participants helped to mitigate individual biases and enrich the evaluation process.
 
As for the reviewer’s third concern, we appreciate your suggestion to consider analyzing inter-rater variability in the evaluation process. However, in our study, participants were tasked with distinguishing between machine learning-generated (MLG) and real surgical outcome (RSO) images, with specificity, sensitivity, and precision values calculated for each group of participants (engineers and medical professionals). Additionally, a McNemar test was conducted to analyze the participants' ability to differentiate between MLG and RSO images. Given the focus on participants' individual responses and the calculation of performance metrics for each group, such as specificity, sensitivity, and precision, we believe that these analyses provide a comprehensive assessment of the participants' ability to differentiate between MLG and RSO images. The McNemar test further evaluated the differences in responses between the groups. Considering the nature of our study design and the specific analyses conducted to evaluate participants' performance in distinguishing between the image types, we find that performing statistics for inter-rater variability may not be necessary in this context. We appreciate your feedback and the consideration of additional analyses.
\end{revresponse}

\begin{revcomment}
Incomplete Explanation of Data Augmentation: The data augmentation method used in this study modifies the lower face while keeping the upper face unchanged.

Problem: It is unclear how realistic these augmented samples are.
The study does not test whether augmentation improves real-world prediction accuracy beyond synthetic datasets.

Recommendation: Provide qualitative examples showing before-and-after augmentation effects.
Conduct a control experiment comparing model performance with and without augmentation on real patient data.
\end{revcomment}

\begin{revresponse}
    First, there seems to be a misunderstanding regarding our data augmentation approach. Contrary to your description, we modify the upper face while keeping the lower face unchanged. The lower face is directly copied from real patient data, ensuring its realism and mitigating concerns about unrealistic augmented samples.

Second, our ablation study already includes an experiment evaluating the impact of data augmentation on model performance using real patient data. Please refer to the last row of Figure 5 and the last row of Table 6 for the detailed comparison. 
\end{revresponse}

\begin{revcomment}
    Lack of Direct Comparison to Commercial Virtual Surgical Planning (VSP) Tools: The study claims that its method outperforms commercial VSP software, but no direct comparison to Dolphin 3D, Morpheus 3D, or 3dMD Vultus is provided.
    
Problem: Without benchmark comparisons, it is unclear whether the proposed approach is truly superior.

- Recommendation: Include a direct side-by-side evaluation using commercial software.
Discuss the trade-offs between automation and clinical accuracy.

\end{revcomment}

\begin{revresponse}[]
VSP is not designed for automated prediction; instead, solutions like Dolphin 3D, Morpheus 3D, or 3dMD Vultus rely on manual, human-involved planning. In contrast, our method provides an automated prediction tool that streamlines the process by eliminating the need for additional CBCT imaging.

Unlike VSP systems, which typically require human annotations, our approach operates without manual intervention. A direct comparison with VSP systems is beyond the scope of this work.

\end{revresponse}
\begin{revcomment}
     Overreliance on Chamfer and Hausdorff Distances: Chamfer Distance and Hausdorff Distance are mathematical metrics that do not fully capture perceived aesthetic and functional outcomes.
     
A lower Hausdorff Distance does not guarantee a visually natural or surgically ideal result.

Recommendation: Use additional clinical shape-based metrics (e.g., facial profile angle, lip prominence, symmetry indices).
\end{revcomment}

\begin{revresponse}[]
Thank you for raising this important point.

We agree that a lower Hausdorff Distance does not directly correlate with the visual or functional ideality of a surgical outcome. However, the Hausdorff Distance serves as a strong metric for measuring geometric accuracy between predicted and real faces, which is a key factor in ensuring that the model can predict realistic facial appearance.

While it’s true that these metrics alone don’t fully capture the aesthetic or functional outcomes, they offer a solid foundation for assessing the model’s alignment with realistic anatomical structures. In our study, we complement these geometric metrics with user studies to evaluate the visual naturalness and clinical suitability of the predicted results, ensuring a more comprehensive assessment.

Therefore, the Hausdorff Distance, in combination with user studies, helps us show that the model is performing well in terms of geometry, which is a necessary precursor for achieving a clinically acceptable and visually natural result. We plan to expand on this with additional clinical shape-based metrics in future work.
\end{revresponse}

\begin{revcomment}
    


Training Data Split and Cross-Validation Concerns: The study uses 5-fold cross-validation but does not specify how patients were divided.

Problem: If pre- and post-surgery pairs from the same patient are split across training and testing, the model may learn patient-specific features rather than generalizable surgical changes.

Recommendation: Clearly state whether patient data were strictly separated between training and testing.
Consider using a leave-one-patient-out validation approach.
\end{revcomment}

\begin{revresponse}[]

Thank you for your feedback. 

Let me explain the 5-fold cross-validation process in detail:
First, the dataset is shuffled randomly and split into five equally sized groups. For each iteration, one group is held out as the test set, while the remaining four groups are used as the training set. A model is then trained on the training set and evaluated on the test set, with the evaluation score recorded while the trained model is discarded. This process repeats for each group, ensuring every data point is used for validation once. Finally, the overall model performance is summarized by aggregating the evaluation scores across all iterations.



To clarify, in 5-fold cross-validation process, we train five separate models rather than repeatedly training a single model~\cite{manual2013introduction}.



To address the concern, we would like to emphasize that the pre- and post-surgery pairs from the same patient were not split across training and testing. We ensured that each patient's data was strictly kept within either the training or the testing set for each fold, preventing any overlap between the training and test sets for a given patient. This avoids the model from learning patient-specific features that could affect generalizability.
    
\end{revresponse}

==> reviewers/R2_2.tex <==
% Reviewer 2

\stepcounter{reviewer@counter}
\reviewer

\begin{revcomment}
Clarify Subjective Evaluation Limitations: While your user study shows that participants had difficulty distinguishing between machine-generated and real surgical outcomes, please include {an acknowledgment} that this subjective measure—despite its value—does not entirely validate clinical accuracy. A brief note in the discussion addressing potential limitations of relying solely on subjective evaluation, and a suggestion for future work that incorporates additional clinical metrics, would strengthen the manuscript.
        
\end{revcomment}
\begin{revresponse}[]

We appreciate the reviewer's feedback on the limitations of subjective evaluation in our study, especially in light of the results indicating similar performance between engineers and medical professionals in distinguishing between MLG faces and RSO. Noteworthily, despite the value of the subjective measure employed in our study, it is essential to acknowledge that subjective evaluation alone may not entirely validate clinical accuracy. Accordingly, it has been acknowledged in the revised manuscript.

\begin{changes}
Noteworthily, although the subjective measure employed in this study holds value in assessing participants' ability to differentiate between MLG faces and RSO, it is important to acknowledge that subjective evaluation alone may not entirely validate clinical accuracy.
\end{changes}

As for the second part of reviewer’s concern, given the comparable performance of engineers and medical professionals in our study, we acknowledge the importance of incorporating additional objective clinical metrics to complement the subjective evaluations. While the subjective assessment provided valuable insights into the perceptual differences between MLG and RSO, the inclusion of quantitative measures such as cephalometric analyses and facial landmark tracking could offer a more robust validation of orthognathic treatment predictions based on facial surgery outcomes.

Future studies can integrate additional objective clinical metrics alongside subjective evaluations to enhance the validation of orthognathic treatment predictions based on facial surgery outcomes. By incorporating quantitative measures such as cephalometric analyses, facial landmark tracking, and patient-reported outcomes, future research can provide a more comprehensive assessment and validation of machine learning-generated facial predictions in the context of orthognathic surgery. As suggested this part has been included in the discussion section of the revised manuscript.

\begin{changes}
    Finally, while the subjective evaluation provided insights into the perceptual differences between MLG faces and RSO, it is crucial to recognise the limitations of relying solely on subjective assessments. Subjective measures, by nature, may introduce bias and subjective interpretation, potentially affecting the overall validity and reliability of the study findings. To mitigate these limitations, future studies can integrate quantitative clinical metrics and objective measures to complement subjective assessments, enhancing the study outcomes' validity and reliability. Incorporating quantitative measures such as cephalometric analyses, facial landmark tracking, and patient-reported outcomes will facilitate a more comprehensive assessment and validation of machine learning-generated facial predictions in the context of orthognathic surgery.
\end{changes}


\end{revresponse}

\begin{revcomment}
Enhance Explanation on Data Augmentation: Although your response clarifies that the augmentation modifies the upper face (not the lower), consider adding a short qualitative example or figure that directly illustrates the "before-and-after" effect. This will help readers better visualize how your augmentation method contributes to improved prediction accuracy.
\end{revcomment}
\begin{revresponse}[]

Thank you for your valuable suggestion regarding the need to enhance the explanation of data augmentation in our study. 
%We appreciate your attention to this aspect and your interest in visualizing the impact of our augmentation method on prediction accuracy.

We've included an ablation study of data augmentation, which shows both quantitative and qualitative results. Specifically, the quantitative results are presented in the last row of Table 6, while the qualitative results can be found in the last row of Figure 5 in the manuscript.

To make this point clearer, we have revised the “Data augmentation” section of the manuscript, where we now reference these experiments explicitly. 

\begin{changes}
To evaluate the impact of data augmentation, we conducted an ablation study, with the results presented in the last row of Table 6 and the last row of Figure 5.
\end{changes}




    
\end{revresponse}

\begin{revcomment}
Highlight Limitations and Future Work: In the revised manuscript, it would be beneficial to explicitly state the limitations of your study—such as the dataset being limited to Asian patients and the exclusion of long-term skeletal changes—and mention plans for future research to address these aspects.
\end{revcomment}

\begin{revresponse}[]
Thank you for your feedback on highlighting the limitations of our study and addressing future work in the revised manuscript. We have explicitly stated the limitations, including the dataset being limited to Asian patients and the exclusion of long-term skeletal changes in the “Limitation” section of the revised manuscript. To address these limitations, we plan to expand the dataset's diversity in future research and continue monitoring potential long-term changes. These updates aim to enhance the study's applicability and reliability. 

\end{revresponse}


